Connected but Late: Sample Age of Commercial BLE Wearables under Wi-Fi Coexistence for Real-Time Clinical Applications

Wearable sensors are increasingly being used in real-time clinical applications, such as rehabilitation robots and live therapy monitoring. As Healthcare 5.0 moves towards personalized therapies, their use will continue growing, potentially compromising communication reliability. Most wearables transmit over Bluetooth Low Energy, sharing 2.4 GHz with institutional Wi-Fi. Previous coexistence studies have focused on whether data arrive, rather than when. We measured sample age for a commercial electrocardiogram strap, from acquisition through the gateway to storage in our platform MEDWEAR, in an anechoic chamber and a hospital rehabilitation gym, and we compared it with illustrative clinical deadlines. Without load, the strap's own framing was the largest source of delay, making samples on average 280 ms and up to 550 ms old before transmission. Wi-Fi load had no measurable effect while adaptive frequency hopping could avoid the loaded channel. In a stress test, which forced the link onto the loaded channel, the link became the dominant source of delay, adding up to 11 s. The link stayed connected, but a median of 29% of samples and up to 98% (worst case) were older than 1 s on arrival at the gateway. The gym behaved mostly like the quiet chamber, but during one traffic burst, while hopping was restricted, up to 4.6% of samples were older than 1 s. These results show that a connected link can deliver late data. Therefore, sensors intended for real-time clinical applications should be profiled in situ and monitored based on sample age rather than connection status alone.

==> supplabels.tex <==
\makeatletter
\@namedef{r@S-sup:platform}{{S1}{1}{}{}{}}
\@namedef{r@S-fig:s-architecture}{{S1}{1}{}{}{}}
\@namedef{r@S-tab:s-roles}{{S1}{1}{}{}{}}
\@namedef{r@S-sup:streaming}{{S1-D}{1}{}{}{}}
\@namedef{r@S-sup:chamber}{{S2}{1}{}{}{}}
\@namedef{r@S-tab:s-ledger}{{S2}{2}{}{}{}}
\@namedef{r@S-sup:instruments}{{S2-A}{2}{}{}{}}
\@namedef{r@S-fig:s-maps}{{S2}{2}{}{}{}}
\@namedef{r@S-tab:s-conditions}{{S3}{3}{}{}{}}
\@namedef{r@S-tab:s-link}{{S4}{3}{}{}{}}
\@namedef{r@S-tab:s-zeroheadroom}{{S5}{3}{}{}{}}
\@namedef{r@S-sup:sensitivity}{{S2-F}{3}{}{}{}}
\@namedef{r@S-tab:s-sensitivity}{{S6}{4}{}{}{}}
\@namedef{r@S-sup:gym}{{S3}{4}{}{}{}}
\@namedef{r@S-fig:s-perrun}{{S3}{4}{}{}{}}
\@namedef{r@S-sup:replay}{{S4}{4}{}{}{}}
\@namedef{r@S-fig:s-load}{{S4}{5}{}{}{}}
\@namedef{r@S-tab:s-replay-steps}{{S7}{5}{}{}{}}
\@namedef{r@S-tab:s-replay-window}{{S8}{5}{}{}{}}
\@namedef{r@S-sup:benchmark}{{S5}{5}{}{}{}}
\makeatother

